Creation and evaluation of timelines for longitudinal user posts

There is increasing interest to work with user generated content in social media, especially textual posts over time. Currently there is no consistent way of segmenting user posts into timelines in a meaningful way that improves the quality and cost of manual annotation. Here we propose a set of methods for segmenting longitudinal user posts into timelines likely to contain interesting moments of change in a user's behaviour, based on their online posting activity. We also propose a novel framework for evaluating timelines and show its applicability in the context of two different social media datasets. Finally, we present a discussion of the linguistic content of highly ranked timelines.

==> sections/z_Optional_Sections.tex <==
\subsection{Comparison to Baselines}

In this section we compare our timeline generation method on different baseline datasets, and we also compare with more traditional evaluation setups, namely covering score and F1 scores.

\subsubsection{Suicide Ideation Detection Datasets}

There is a lack of freely available social media datasets containing human-labelled annotations indicating changes in mental health conditions. Previous work such as \cite{mishra_snap-batnet_2019} involves first creating timelines based on the presence of keywords that are within a lexicon that was identified to suggest suicidal intent, similar to the baseline timeline generation method we have presented as our "keywords" methods in \ref{tab: summed votes}. While such an approach will likely produce several annotations of changes in mental health, this approach suffers from biasing the linguistic content of the annotated dataset - restricting the content of the dataset to contain posts containing words within the lexicon - biasing downstream work (e.g. models trained on this dataset) to this lexicon. We therefore experiment in this section with our timeline generation approach, which is blind to linguistic content, on creating timelines indicating \emph{suicide intent} rather than Moments of Change.

The work of \cite{mishra_snap-batnet_2019} identifies candidate MoCs by first identifying posts that have the presence of keywords in a lexicon expressing suicide intent. Candidate timelines are then created around these, by extracting the previous $n \leq 100$ posts (if they exist) for that user, as an unlabelled timeline. To reduce annotation cost, the authors only provide the candidate MoC to the annotators, as a post to be annotated and therefore the timelines are not annotated on a longitudinal basis (i.e. annotations are only made on the post level, rather than taking into account the surrounding temporal context). The historical context is included in the dataset as unlabelled data, to be used for unsupervised learning of the associated user. While the authors report a dataset with a reasonable density of posts labelled with suicide intent (roughly 20\%), we expect this candidate timeline creation can be improved in a few ways. Firstly, only single posts are provided to annotators to be labelled. However different users have different expressions of suicide intent, and taking into account the user's surrounding posts can help \emph{annotators} better assess the presence of suicide intent - based on the user's identified baseline and disposition and achieve fewer false positives. Additionally, posts may not clearly express suicide intent unless taking into account their previous and future posts (e.g. they may simply be singing a song lyric or joking, which could be made more clearly if annotators see they have a history of doing so). Even if the entire timeline is provided to annotators, and assessed on a longitudinal basis there are still problems with their candidate timeline creation approach. Namely, only the historical context would be provided to the annotators (i.e. the previous 100 posts) relative to the candidate MoC. We expect that providing both historical \emph{and future} context around the candidate MoC will help annotators better distinguish different types \emph{changes} (e.g. switches/ escalations as described in \cite{anonymous}) in a user's profile, and therefore more easily identify anomalous posts indicating suicide intent, based on the baseline of the user both before and after the post which was identified as a candidate MoC. Furthermore, even if the candidate timelines are to be unlabelled - we expect that providing future and historical context can improve the performance of downstream unsupervised models if they take both contexts into account. We therefore experiment with using our candidate timeline creation approach described in \ref{sec: timeline creation} which includes both historical and future context as a radius around candidate MoCs.

\subsubsubsection{Results}


\subsubsection{Conventional Evaluation Setups}

In this paper we have introduced a novel evaluation approach for assessing the ability of timeline generation approaches for creating timelines that will subsequently be annotated with a high density of the rare labels of interest (i.e. moments of change). We experiment in this section to show how this evaluation setup compares to more traditional evaluation approaches, namely those using covering and F1 scores. 

Evaluating changes in sequence data is itself a challenging task, and has been explored recently in a review by \cite{van2020evaluation}. The authors express that covering and F1 scores should be adopted for evaluating the performance of models capability of identifying the presence of changes in sequence data. In this context, we treat the human annotators as models, and assess whether they are able to identify such changes using their proposed evaluation metrics - and treat their assessments as ground-truth.

Another inherent challenging problem with evaluating changes in sequence data is that disagreements between annotators can be very common, and integrating such noisy annotations and assessing models against this noise is another challenge that needs to be addressed. This is still a fairly open research area and is the focus of several recent works \cite{uma_semeval-2021_2021, simpson_low_2020, paun_aggregating_2021, fornaciari_beyond_2021}. For this work, we follow the a simple aggregation approach used in \cite{anonymous} which involves taking .... 

\subsubsubsection{Results}


